A Possible Mechanism for Overcoming the Electrostatic Barrier Against Dust Growth in Protoplanetary disks

The coagulation of dust particles under the conditions in protoplanetary disks is investigated. The study focuses on the repulsive electrostatic barrier against growth of charged dust grains. Taking into account the photoelectric effect leads to the appearance of a layer at intermediate heights where the dust has a close to zero charge, enabling the dust grains to grow efficiently. An increase in the coagulation rate comes about not only due to the lowering of the Coulomb barrier, but also because of the electrostatic attraction between grains of opposite charge due to the non-zero dispersion of the near-zero charge. Depending on the efficiency of mixing in the disk, the acceleration of the evolution of the dust in this layer could be important, both in the quasi-stationary stage of the disk evolution and during its dispersal.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%               Macros for TeX/LaTeX documents
%
% Author: Frank C. van den Bosch
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etal}{{et al.~}}

\newcommand{\kmsmpc}{\>{\rm km}\,{\rm s}^{-1}\,{\rm Mpc}^{-1}}
%\newcommand{\kms}{\>{\rm km}\,{\rm s}^{-1}}
%\newcommand{\pc}{\>{\rm pc}}
\newcommand{\cm}{\>{\rm cm}}
\newcommand{\Mpc}{\>{\rm Mpc}}
\newcommand{\kpc}{\>{\rm kpc}}
\newcommand{\Msun}{\>{\rm M_{\odot}}}
\newcommand{\Lsun}{\>{\rm L_{\odot}}}
\newcommand{\MLsun}{\>({\rm M}/{\rm L})_{\odot}}
\newcommand{\Mbh}{M_{\bullet}}
\newcommand{\Vrot}{V_{\rm rot}}
\newcommand{\mtol}{\>{\rm (M/L)_{\odot}}}
\newcommand{\erg}{\>{\rm erg}}
\newcommand{\kpch}{\>{h^{-1}{\rm kpc}}}
\newcommand{\mpch}{\>h^{-1}{\rm {Mpc}}}
\newcommand{\yr}{\>{\rm yr}}
\newcommand{\yrs}{\>{\rm yrs}}
\newcommand{\Msunh}{\>h^{-1}\rm M_\odot}
\newcommand{\Lsunh}{\>h^{-2}\rm L_\odot}
\newcommand{\calN}{{\cal N}}
\newcommand{\wcalN}{\tilde{{\cal N}}}
\newcommand{\walpha}{\tilde{\alpha}}
\newcommand{\wLstar}{\tilde{L}^{*}}
\newcommand{\hxi}{\hat{\xi}}
\newcommand{\lamA}{${\Lambda}30/90 \, $}
\newcommand{\lamC}{${\Lambda}25/75 \, $}
\newcommand{\lamD}{${\Lambda}20/65 \, $}
\newcommand{\lamB}{${\Lambda}30/65 \, $}
\newcommand{\reference}{\bibitem}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\vcir}{V_{\rm c}}
\newcommand{\vh}{V_{\rm c}}
\newcommand{\Obaryon}{{\Omega_{\rm B,0}}}
\newcommand{\Kdegree}{\>{\rm K}}
\newcommand{\keV}{\>{\rm keV}}
\newcommand{\vhalo}{V_{\rm c}}
\newcommand{\Tvir}{T_{\rm vir}}
\newcommand{\rmd}{{\rm d}}
\newcommand{\vesc}{V_{\rm esc}}
\newcommand{\Lya}{{\rm Ly}\alpha}
\newcommand{\msunh}{\>h^{-1}\rm M_\odot}
\newcommand{\Lsunhh}{\,h^{-2}\rm L_\odot}
\newcommand{\Msunhh}{\,h^{-2}\rm M_\odot}

%%% 
\newcommand{\lcen}{L}
\newcommand{\msc}{M_{\rm *c}}
\newcommand{\pc}{Q}
\newcommand{\pten}{Q_{\rm 10}}
\newcommand{\lc}{\lcen}
\newcommand{\avg}[1]{\langle #1 \rangle}
\newcommand{\avglogm}{\avg{\log M}(\lcen)}
\newcommand{\avglogmsq}{\avg{(\log M)^2}(L_c)}
\newcommand{\avgloglc}{\avg{\log \lcen}(M)}
\newcommand{\siglogm}{\sigma_{\log M}(\lcen)}
\newcommand{\ploglcm}{P(\log \lcen|M)}
\newcommand{\plogmlc}{P(\log M|\lcen)}
\newcommand{\drm}{{\rm d}}
\newcommand{\pdv}{{P (\Delta V)}}
\newcommand{\dv}{{\Delta V}}
% \newcommand{\sigcen}{\sigma_{\rm cen}}
\newcommand{\siglcen}{\sigma_{\log L}}
\newcommand{\sigcenm}{\sigma_{\log M_*}}
\newcommand{\sigmscen}{\sigma_{\log M_*}}
\newcommand{\sigp}{\sigma_{\log Q}}
\newcommand{\sigcenp}{\sigma_{\log Q}}
\newcommand{\sigsw}{\sigma_{\rm sw}}
\newcommand{\sighw}{\sigma_{\rm hw}}
\newcommand{\sigsat}{\sigma_{\rm sat}}
\newcommand{\avgsigsatsq}{\avg{\sigsat^2}}
\newcommand{\avnsat}{\avg{N_{\rm s}}}
\newcommand{\avnsatm}{\avnsat(M)}
\newcommand{\philcm}{\Phi_{\rm c}(L|M)}
\newcommand{\philsm}{\Phi_{\rm s}(L|M)}
\newcommand{\plcm}{P(\lcen|M)}
\newcommand{\pmscm}{P(\msc|M)}
\newcommand{\pmlc}{P(M|\lcen)}
\newcommand{\pmpc}{P(M|\pc)}
\newcommand{\ppcm}{P(\pc|M)}
\newcommand{\sigav}{\sigma_{\rm av}}
%special
\newcommand{\fr}{f_{\rm r}}
\newcommand{\fb}{f_{\rm b}}
\newcommand{\fint}{f_{\rm int}}
\newcommand{\sigr}{\sigma_{\rm r}}
\newcommand{\sigb}{\sigma_{\rm b}}
\newcommand{\Mr}{M_{\rm r}}
\newcommand{\Mb}{M_{\rm b}}
\newcommand{\Rh}{R_{\rm h}}
\newcommand{\Rs}{R_{\rm s}}
\newcommand{\dvh}{(\dv)_{\rm h}}
\newcommand{\dvs}{(\dv)_{\rm s}}
\newcommand{\Sset}{\hat{S}}
%%%%% less than approximate and all that

\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\prosima{$\; \buildrel \propto \over \sim \;$}
\def\gsim{\lower.7ex\hbox{\gtsima}}
\def\lsim{\lower.7ex\hbox{\ltsima}}
\def\simgt{\lower.7ex\hbox{\gtsima}}
\def\simlt{\lower.7ex\hbox{\ltsima}}
\def\simpr{\lower.7ex\hbox{\prosima}}
\def\la{\lsim}
\def\ga{\gsim}
\def\lta{\la}
\def\gta{\ga}

%%%%%% Useful for editing drafts

\newcommand{\XXX}[2]{{\sf #1}}
\newcommand{\QQQ}[1]{{\sc $<$#1$>$}}

%To return to the original version, comment the previous two lines and
%uncomment the next two lines 

%\newcommand{\XXX}[2]{#2}
%\newcommand{\QQQ}[1]{}

%%%%%% Useful for bibliography

\newcommand{\apj}{ApJ}
\newcommand{\apjl}{ApJL}
\newcommand{\apjs}{ApJS}
\newcommand{\aj}{AJ}
\newcommand{\mnras}{MNRAS}
\newcommand{\aap}{A\&A}
\newcommand{\aaps}{A\&AS}
\newcommand{\araa}{ARA\&A}
\newcommand{\nat}{Nature}
\newcommand{\pasp}{PASP}

%%%%%% Useful measures of length for use with psfig

\newdimen\hssize
\hssize=8.4truecm
\newdimen\hdsize
\hdsize=17.7truecm

%%%%%%

\def\fn#1{$^{\ref{#1}}$}
\def\fit#1{\footnotesize \it #1 }
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

